Poke and Strike: Learning Task-Informed Exploration Policies

In many dynamic robotic tasks, such as striking pucks into a goal outside the reachable workspace, the robot must first identify the relevant physical properties of the object for successful task execution, as it is unable to recover from failure or retry without human intervention. To address this challenge, we propose a task-informed exploration approach, based on reinforcement learning, that trains an exploration policy using rewards automatically generated from the sensitivity of a privileged task policy to errors in estimated properties. We also introduce an uncertainty-based mechanism to determine when to transition from exploration to task execution, ensuring sufficient property estimation accuracy with minimal exploration time. Our method achieves a 90% success rate on the striking task with an average exploration time under 1.2 seconds, significantly outperforming baselines that achieve at most 40% success or require inefficient querying and retraining in a simulator at test time. Additionally, we demonstrate that our task-informed rewards capture the relative importance of physical properties in both the striking task and the classical CartPole example. Finally, we validate our approach by demonstrating its ability to identify object properties and adjust task execution in a physical setup using the KUKA iiwa robot arm.

==> Makefile <==
# Makefile for compiling a *.tex file into a *.pdf file
# The current folder must contain only one *.tex file
#
# Author: Joao Moura
# Email: jmm7@hw.ac.uk
# Last Modified at 01/06/2016
#
#################################################################
#################################################################
# Identify what is the name of the *.tex file to compile
# NOTE: There must be a single *.tex file in the current directory
TEX = pdflatex -shell-escape
# BIB = biber
BIB = bibtex
TIKZ = Tikz
FILE_TEX=$(wildcard *.tex)
FILE_BIB=refs.bib
TARGET=$(FILE_TEX:.tex=)
#################################################################

#################################################################
# Rule that runs whether the make is called or the target file is outdated.
FORCE: $(FILE_TEX)
	$(TEX) $(TARGET)

$(TARGET).bbl: $(FILE_TEX) $(FILE_BIB)
	$(BIB) $(TARGET)

$(TARGET).nlo: $(FILE_TEX)
	makeindex $(TARGET).nlo -s nomencl.ist -o $(TARGET).nls

$(TARGET).glo: $(FILE_TEX)
	makeglossaries $(TARGET)
#################################################################

#################################################################
# Rule to create a bibtex file
.PHONY: gloss
gloss:
	makeglossaries $(TARGET)
#################################################################

#################################################################
# Rule to create a bibtex file
.PHONY: nom
nom:
	makeindex $(TARGET).nlo -s nomencl.ist -o $(TARGET).nls
#################################################################

#################################################################
# Rule to create a bibtex file
.PHONY: bib
bib:
	$(BIB) $(TARGET)
#################################################################

#################################################################
# Rule for cleaning: It removes all the files with TARGET name except the file with *.tex extension
.PHONY: clean
clean: 
	rm -f $(filter-out $(TARGET).tex $(TARGET).bib, $(wildcard $(TARGET).*))
#################################################################

#################################################################
# Rule for cleaning all tikz files
.PHONY: cleanall
cleanall: 
	rm -f $(filter-out $(wildcard tikz/*.tex) $(TARGET).tex $(TARGET).bib, $(wildcard tikz/*.*) $(wildcard $(TARGET).*))
#################################################################

#################################################################
# Rule for cleaning the bib file
.PHONY: cleanbib
cleanbib:
	# Remove unnecessary keywords:
	gsed -i '/^abstract/d' $(FILE_BIB)
	gsed -i '/^archivePrefix/d' $(FILE_BIB)
	gsed -i '/^arxivId/d' $(FILE_BIB)
	gsed -i '/^eprint/d' $(FILE_BIB)
	gsed -i '/^isbn/d' $(FILE_BIB)
	gsed -i '/^issn/d' $(FILE_BIB)
	gsed -i '/^mendeley-tags/d' $(FILE_BIB)
	gsed -i '/^pmid/d' $(FILE_BIB)
	gsed -i '/^primaryClass/d' $(FILE_BIB)
	gsed -i '/^keywords/d' $(FILE_BIB)
	gsed -i '/^url/d' $(FILE_BIB)
	gsed -i '/^file/d' $(FILE_BIB)
	gsed -i '/^month/d' $(FILE_BIB)
	# Insert tab before keyword:
	gsed -i 's/^\([a-z]\)/\t\1/' $(FILE_BIB)
	# Remove double brackets in titles:
	gsed -i 's/{{\(.*\)}}/{\1}/' $(FILE_BIB)
	# Add a line after each reference:
	gsed -i '/^}/a\\' $(FILE_BIB)
#################################################################

